A Comparative Study of the Streaming Instability: Unstratified Models with Marginally Coupled Grains

The streaming instability is a leading mechanism for concentrating solids and initiating planetesimal formation in protoplanetary disks. Although numerous studies have explored its linear growth, nonlinear evolution, and implications for planet formation, the diversity of numerical methods and dust treatments used across the literature has made it difficult to assess which features of the instability are physically robust and which arise from code-dependent choices. We present the first systematic comparison of seven hydrodynamic codes--spanning finite-volume and finite-difference schemes and modeling dust either as Lagrangian particles or as a pressureless fluid--applied to the unstratified streaming instability with a dimensionless stopping time of unity. All codes reproduce the characteristic sequence of exponential growth, filament formation, and turbulent saturation, demonstrating broad agreement in the qualitative behavior of the instability. Quantitatively, however, the dust model remains the dominant source of variation at moderate resolution: particle-based simulations reach higher peak densities and exhibit broader high-density tails than fluid-based models at $512^2$ resolution, although increasing the number of particles brings their initial maximum density evolution into close agreement with that of dust-fluid models. At $1024^2$, these differences diminish substantially, indicating better agreement of the saturated-state statistics across dust treatments. In terms of computational performance, most particle implementations suffer from imbalanced parallelized loads, while execution on a GPU is at least two to three times more energy efficient and scales better at higher resolutions than on CPUs. Given the intrinsic stochasticity of this nonlinear system, only statistical diagnostics remain meaningful across codes.

==> preamble.tex <==
\usepackage{apjfonts}

\usepackage{graphicx}
\usepackage{color}

\usepackage{amsbsy}
\usepackage{mathrsfs}
\usepackage{mathpazo}
\usepackage{bm}
\usepackage{amsmath}
%\usepackage{amssymb}

\usepackage{xfrac}
\usepackage{sidecap}
%\usepackage{setspace}
%\singlespacing
\usepackage{url}
\usepackage{hyperref}
\usepackage{enumitem}
%\usepackage{natbib}

%\usepackage{ulem}
%\usepackage{rotating, lscape, longtable}
%\usepackage{wrapfig}
%\usepackage{esint}
%\usepackage{wasysym}

%\newlength{\hfwidth}
%\newlength{\hfwidthsingle}
%\addtolength{\hfwidthsingle}{.5\textwidth} %single fig in figure\fig
%\addtolength{\hfwidth}{.497\textwidth} %single fig in figure*
\newlength{\figspace}
\addtolength{\figspace}{-4mm} %for reducing space between figures and their captions


\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\pderiv}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\deriv}[2]{\frac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}
\newcommand{\pderivn}[3]{\frac{{\partial{}}^{#3}{#1}}{{\partial{#2}}^{#3}}}
\newcommand{\aderiv}[1]{\frac{\mathrm{D}{#1}}{\mathrm{D}t}}
\newcommand{\ptderiv}[1]{\frac{\partial{#1}}{\partial{t}}}
\newcommand{\ee}{\mathrm{e}}
\newcommand{\kderiv}[1]{\frac{{\mathcal D} #1}{{\mathcal D}t}}

\newcommand{\Ma}{\mathrm{Ma}}
\newcommand{\Rey}{\mathrm{Re}}
\newcommand{\Kn}{\mathrm{Kn}}
\newcommand{\Ro}{\mathrm{Ro}}
\newcommand{\St}{\mathrm{St}}
\newcommand{\Sc}{\mathrm{Sc}}
\newcommand{\Stp}{\mathrm{St_p}}

\newcommand{\ttimes}[1]{10^{#1}}
\newcommand{\xtimes}[2]{#1\times{10^{#2}}}
\newcommand{\xstimes}[3]{(#1{\pm}#2) \times 10^{#3}}
\newcommand{\vt}[1]{\boldsymbol{\mathrm{#1}}}       %for tensors
\renewcommand{\v}[1]{{\boldsymbol{#1}}} %for vectors
\renewcommand{\ss}[1]{\scriptsize{#1}}
\newcommand{\tn}[1]{\tiny{#1}}
\newcommand{\ksi}{\xi}
\newcommand{\wdash}{\white{-}}

\newcommand{\del}{\v{\nabla}}
\newcommand{\grad}{\del}
\newcommand{\Div}{\del\cdot}
\newcommand{\curl}{\del\times}
\newcommand{\Laplace}{\nabla^2}
\newcommand{\de}{\mathrm{d}} 
\newcommand{\rint}{$s_{\rm int}\,$}
\newcommand{\rext}{$s_{\rm ext}\,$}
\newcommand{\hatr}{\hat{\v{r}}}
\newcommand{\hattht}{\hat{\v{\theta}}}
\newcommand{\hatR}{\hat{\v{R}}}
\newcommand{\hatn}{\hat{\v{n}}}
\newcommand{\hatphi}{\hat{\v{\phi}}}
\newcommand{\hatz}{\hat{\v{z}}}
\newcommand{\haty}{\hat{\v{y}}}
\newcommand{\hatx}{\hat{\v{x}}}

\newcommand{\hatu}{\hat{\v{u}}}
\newcommand{\hatv}{\hat{\v{\varv}}}
\newcommand{\hatw}{\hat{\v{w}}}

\newcommand{\va}{v_{_{\rm A}}}
%\newcommand{\deg}{\ensuremath{^\circ}}
\newcommand{\degreep}{\ensuremath{^\circ}~}
\newcommand{\Msun}{M_\odot}
\newcommand{\msun}{\Msun}
\newcommand{\sun}{\odot}
\newcommand{\Eps}{{\rm Eps}}
\newcommand{\dv}{\Delta{\v{v}}}
\newcommand{\mearth}{\,$M_{\oplus}$}
\newcommand{\mearthp}{\,$M_{\oplus}$ }
\newcommand{\rearth}{\,$R_{\oplus}$}
\newcommand{\rearthp}{\,$R_{\oplus}$ }
\newcommand{\mps}{m\,s$^{-1}$}
\newcommand{\vrms}{$v_{\rm rms}$} 
\newcommand{\vmax}{$v_{\rm max}$} 
\newcommand{\vesc}{$v_{\rm esc}$} 
\newcommand{\mdot}{\dot{m}} 
\newcommand{\cv}{c_{_{V}}}
\newcommand{\cp}{c_p}
\newcommand{\tauc}{\tau_{\rm cool}}
\newcommand{\taus}{\tau_{\rm stop}}
\newcommand{\cs}{c_\mathrm{s}}
\newcommand{\csO}{c_\mathrm{s0}}
\newcommand{\Mjup}{\,M_\mathrm{J}}  %mm modified M_{Jup} -> M_J
\newcommand{\alphat}{\beta}
\newcommand{\tauref}{\tau_0}

%for the table
\newcommand{\cte}{\small const}
\newcommand{\mm}[2]{#1{\tiny$\pm$#2}}

\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[2]{Eqs.~(\ref{#1})~and~(\ref{#2})}
\newcommand{\Eqss}[2]{Eqs.~(\ref{#1})--(\ref{#2})}
\newcommand{\eq}[1]{\Eq{#1}}
\newcommand{\eqp}[1]{(Eq.~\ref{#1})}
\newcommand{\eqs}[2]{\Eqs{#1}{#2}}
\newcommand{\eqss}[2]{\Eqss{#1}{#2}}
\newcommand{\App}[1]{Appendix~\ref{#1}}
\newcommand{\app}[1]{\App{#1}}
\newcommand{\Figure}[1]{Figure~\ref{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Figp}[1]{(Fig.~\ref{#1})}
\newcommand{\fig}[1]{\Fig{#1}}
\newcommand{\figp}[1]{\Figp{#1}}
\newcommand{\Figs}[2]{Figs.~\ref{#1}~and~\ref{#2}}
\newcommand{\Figss}[2]{Figs.~\ref{#1}--\ref{#2}} 
\newcommand{\figs}[2]{\Figs{#1}{#2}}
\newcommand{\figss}[2]{\Figss{#1}{#2}}
\newcommand{\Table}[1]{Table~\ref{#1}}
\renewcommand{\table}[1]{Table~\ref{#1}}
\newcommand{\sect}[1]{Sect.~\ref{#1}}

\newcommand{\rhoagn}{\rho_{_{\rm AGN}}}

\newcommand{\lla}{\left\langle}
\newcommand{\rra}{\right\rangle}

%colors for editting
\definecolor{brown}{rgb}{0.42,0.24,0.07}
\definecolor{darkgreen}{rgb}{0.0,0.6,0.00}
\definecolor{purple}{rgb}{0.7,0.0,0.7}
\definecolor{black}{rgb}{0.0,0.0,0.0}
\def\red#1{\textcolor{red}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\green#1{\textcolor{darkgreen}{#1}}
\def\brown#1{\textcolor{brown}{#1}}
\def\purple#1{\textcolor{purple}{#1}}
\def\white#1{\textcolor{white}{#1}}
\def\black#1{\textcolor{black}{#1}}

\newcommand{\comm}[1]{\brown{{\it #1}}}

\def\apj{\rm ApJ}
\def\apjl{\rm ApJL}
\def\apjs{\rm ApJS}
\def\aj{\rm AJ}
\def\mnras{\rm MNRAS}
\def\nat{\rm Nature}
\def\pasj{\rm PASJ}
\def\pasp{\rm PASP}
\def\aap{\rm A\&A}
\def\aaps{\rm A\&AS}
\def\apss{\rm APSS}
\def\araa{\rm ARA\&A}
\def\icarus{\rm Icarus}
\def\qjras{\rm QJRAS}
\def\ssr{\rm SSR}
\def\zap{\rm ZAp}
\def\jrasc{\rm Journ.~Royal~Astron.~Soc.~of~Canada}
\def\bain{\rm Bul.~Astron.~Inst.~Netherlands}
\def\baas{\rm Bul.~American~Astron.~Soc.}
\def\prl{\rm Phys.~Rev.~Lett.}
\def\planss{\rm Planet. Space Sci.}
\def\prd{\rm Phys.~Rev.~D}

\newcommand{\eg}{{\it e.g.},~}
\newcommand{\ie}{{\it i.e.},~}
\newcommand{\etal}{{\it et al.}~}

\newcommand{\gsim}{\gtrsim}
\newcommand{\lsim}{\lesssim}

\newcommand{\Mstar}{\ensuremath{M_\star}}
\newcommand{\Lstar}{\ensuremath{L_\star}}
\newcommand{\Lsun}{\ensuremath{L_\odot}}

\newcommand{\hatq}{\hat{\v{q}}}
\newcommand{\hath}{\hat{\v{h}}}
\newcommand{\hate}{\hat{\v{e}}}

\newcommand{\mean}[1]{\left\langle #1 \right\rangle}
\newcommand{\sinf}{\sin{f}}
\newcommand{\cosf}{\cos{f}}
\newcommand{\sinfw}{\sin{\left(f-\omega\right)}}
\newcommand{\cosfw}{\cos{\left(f-\omega\right)}}
\newcommand{\cosE}{\cos{E}}
\newcommand{\teff}{\tau_{\rm eff}}
\newcommand{\hatX}{\hat{\v{X}}}
\newcommand{\hatY}{\hat{\v{Y}}}
\newcommand{\hatZ}{\hat{\v{Z}}}

\newcommand{\sinI} {\sin{I}}
\newcommand{\cosI} {\cos{I}}
\newcommand{\cosO}{\cos{\Omega}}
\newcommand{\sinO}{\sin{\Omega}}
\newcommand{\sinw}{\sin{\omega}}
\newcommand{\cosw}{\cos{\omega}}

\newcommand{\sinisq}{\sin^2{I}}
\newcommand{\sintwow}{\sin{2\omega}}
\newcommand{\costwow}{\cos{2\omega}}
\newcommand{\sintwop}{\sin{2\Psi}}
\newcommand{\costwop}{\cos{2\Psi}}


\newcommand{\hmin}{h_{\rm min}}
\newcommand{\hmax}{h_{\rm max}}
\newcommand{\degree}[3]{{#1}\deg{#2}\min{#3}\sec}
\newcommand{\hour}[3]{{#1}{\rm h}\,{#2}{\rm m}\,{#3}{\rm s}}

\renewcommand{\mod}{\ {\rm mod} \ }

\renewcommand{\deg}{^\circ}
\renewcommand{\min}{^\prime}
\renewcommand{\sec}{^{\prime\prime}}


\newcommand{\boltz}{{\rm exp}\left(h\nu/kT \right)}
\newcommand{\boltzm}{{\rm exp}\left(h\nu_M/kT \right)}

\newcommand{\atom}[2]{$^{#2}${#1}}
\newcommand{\qatom}[2]{^{#2}{\rm #1}}

\newcommand{\const}{\rm const}

\newcommand{\advec}{\v{u}\cdot\del}

